Can Neural Decompilation Assist Vulnerability Prediction on Binary Code?

Vulnerability prediction is valuable in identifying security issues efficiently, even though it requires the source code of the target software system, which is a restrictive hypothesis. This paper presents an experimental study to predict vulnerabilities in binary code without source code or complex representations of the binary, leveraging the pivotal idea of decompiling the binary file through neural decompilation and predicting vulnerabilities through deep learning on the decompiled source code. The results outperform the state-of-the-art in both neural decompilation and vulnerability prediction, showing that it is possible to identify vulnerable programs with this approach concerning bi-class (vulnerable/non-vulnerable) and multi-class (type of vulnerability) analysis.

==> tex/abstract.tex <==
\begin{abstract}
Vulnerability prediction is valuable in identifying security issues efficiently. The most popular solutions and techniques for vulnerability prediction require the source code of the target software system, which is a restrictive hypothesis. Recently, several approaches based on binary code analysis have emerged, showing promising results. However, these solutions lift the binary to formal representations (e.g., disassembled code, LLVM IR, intermediate representation), which fail to bridge the semantic gap between binary and source code, leading to weak performance in vulnerability identification.
This paper presents an explorative study to predict vulnerabilities in binary code without source code or complex representations of the binary, leveraging the pivotal idea of decompiling the binary file through \textit{neural decompilation} and predicting vulnerabilities through deep learning on the decompiled source code. The results outperform the state-of-the-art in both neural decompilation and vulnerability prediction, showing that it is possible to identify vulnerable programs with this approach concerning bi-class (vulnerable/non-vulnerable) and multi-class (type of vulnerability) analysis.
\end{abstract}

%which require a deep knowledge of the high-level language and the target architecture, with a relevant \textit{engineering} effort.

%\vittorio{Il paper presents uno studio sperimentale sulla vulnerability prediction a partire dal binario (senza sorgente disponibile) applicando approccio innovative di Neural Decompilation}


==> tex/lessons.tex <==
% Lessons Learned:
The results of the experimental study provided us with several lessons learned about using neural decompilation in the cybersecurity landscape.  

%\vspace{1pt}
\noindent
\textbf{Applicability of neural decompilation to cybersecurity}.
The idea of leveraging neural decompilation for cybersecurity-related tasks is promising. Specifically, given the quality of the translated code, neural decompilation showed great potential for vulnerability prediction, with the possibility to unlock several novel applications, e.g., binary malware recognition. 
We analyzed three state-of-the-art models, i.e., fairseq, CodeBERT, and CodeT5+, with fairseq emerging as the best-performing model, achieving quality translations comparable to other studies in code translation and providing a representative basis for our experiments.
Future work includes integrating additional models for neural decompilation, with a deeper inspection of pre-trained NMT models.

%\vspace{1pt}
\noindent
\textbf{Use of DL for vulnerability prediction}.
The results of the vulnerability prediction task revealed that DL models were indeed appropriate for vulnerability detection and identification, with transformer-based models emerging as the best performing. The selected models could accurately predict whether a C/C++ function was vulnerable and the related vulnerability in the MITRE CWE taxonomy. 

\begin{comment}

\vspace{1pt}
\noindent
\textbf{Language dependence}.
We do not perform experiments using other high-level (target) or low-level (source) languages but focus on the specific, common case of C/C++ and the x86 architecture. However, we note that the work does not aim to prove the retargetability of the decompilation system but to represent the ease with which a decompiler can be implemented bypassing the knowledge of the specific target and source languages.

\end{comment}

==> tex/table.tex <==

%\begin{table*}[!ht]
%\centering
%\caption{\revision{Network fault models used in the state-of-the-art}}
%\label{tab:related_summary}
%\resizebox{2\columnwidth}{!}{%
%\sffamily 
%\footnotesize 
%\begin{tabular}{|C{4cm}|C{4cm}|C{4cm}|C{4cm}|C{4cm}|C{4cm}|C{4cm}|}
%\hline \textbf{Work} & \textbf{Retargetable} & \textbf{Binary Classification} & \multicolumn{2}{c}{\textbf{Multi-class Classification}} & \textbf{Standardized taxonomy}\\
%\rowcolor{blue!8}



==> tex/threats.tex <==
%\vspace{1pt}
\noindent
\textbf{Dataset}. The chosen dataset, Juliet C/C++ 1.3, is a synthetic dataset, i.e., novel data created from real data with the same statistical properties. Using a synthetic dataset provides a large amount of samples, accurately annotated with ground truth. However, the synthetic data do not perfectly align with actual data regarding the size and complexity of real code. Therefore, the vulnerability detection accuracy on synthetic data may be higher than in real data. This may hinder the external validity of the study. Nevertheless, the synthetic data still allow us to analyze the decompilation task and the prediction of vulnerabilities in the translated code, which represents a good starting point for this research direction. Moreover, it is challenging to find datasets in the literature that satisfy the requirements for vulnerability prediction in binary code, as illustrated in Section \ref{sec:dataset}. Specifically, Juliet represents a fair trade-off between the requirements for the dataset: i) a dataset composed of compilable C/C++ functions and ii) labeled with the vulnerabilities from a standardized taxonomy. 

%\vspace{1pt}
\noindent
\textbf{Models selection}. The selection of transformer-based and DL models for the neural decompilation and vulnerability prediction tasks may impact the study's external validity. On the one hand, we selected three state-of-the-art models, namely fairseq, CodeBERT, and CodeT5+, for neural decompilation performing a comparative study to assess their capabilities for this task.
On the other hand, we leveraged CodeBERT, CodeT5+, CodeGPT, and traditional DL models for vulnerability prediction since they represent the most popular solution for this task \cite{zheng2019recurrent, schaad2023deep, dahl2020stack, chen2023diversevul}. We tried to include, to the best of our knowledge, models with different architectures and capabilities, representative of the state-of-the-art.

%\vspace{1pt}
\noindent
\textbf{Metrics}. To evaluate the performance of neural decompilation, we selected output similarity metrics such as BLEU, METEOR, ED, and ROUGE. This choice may threaten the construct validity since such metrics may not capture the correctness of the decompiled code. Nevertheless, output similarity metrics represent the most popular practice for evaluating NMT models, both for code-to-code (as in similar works on neural decompilation \cite{hosseini2022beyond, katz2018using}) and NL-to-code translation tasks \cite{liguori2023evaluates}. Specifically, ED represents the prevalent metric to estimate the performance of code-to-code translation.  
